SC-Bench: A Large-Scale Dataset for Smart Contract Auditing

There is a huge demand to ensure the compliance of smart contracts listed on blockchain platforms to safety and economic standards. Today, manual efforts in the form of auditing are commonly used to achieve this goal. ML-based automated techniques have the promise to alleviate human efforts and the resulting monetary costs. However, unlike other domains where ML techniques have had huge successes, no systematic ML techniques have been proposed or applied to smart contract auditing. We present SC-Bench, the first dataset for automated smart-contract auditing research. SC-Bench consists of 5,377 real-world smart contracts running on Ethereum, a widely used blockchain platform, and 15,975 violations of standards on Ehereum called ERCs. Out of these violations, 139 are real violations programmers made. The remaining are errors we systematically injected to reflect the violations of different ERC rules. We evaluate SC-Bench using GPT-4 by prompting it with both the contracts and ERC rules. In addition, we manually identify each violated rule and the corresponding code site (i.e., oracle) and prompt GPT-4 with the information asking for a True-or-False question. Our results show that without the oracle, GPT-4 can only detect 0.9% violations, and with the oracle, it detects 22.9% violations. These results show the potential room for improvement in ML-based techniques for smart-contract auditing.

==> figures/erc20-high-prompt.tex <==
Given a solidity function transferFrom and the related parts from a smart contract and an ERC rule.
Whether the function transferFrom and its related parts have the check for the rule? Reply in "YES" or "NO"

Rule:"""
throw unless the \_from account has deliberately authorized the sender of the message via some mechanism.
"""

Function(and related parts) to audit:"""
contract ERC20 is Context, IERC20 {

    function transferFrom(
        address from,
        address to,
        uint256 amount
    ) public virtual override returns (bool) {
        _transfer(from, to, amount);
        return true;
    }

    function _transfer(
        address from,
        address to,
        uint256 amount
    ) internal virtual {
        require(from != address(0), "ERC20: transfer from the zero address");
        require(to != address(0), "ERC20: transfer to the zero address");

        uint256 fromBalance = _balances[from];
        require(fromBalance >= amount, "ERC20: transfer amount exceeds balance");
        unchecked {
            _balances[from] = fromBalance - amount;
            _balances[to] += amount;
        }

        emit Transfer(from, to, amount);

    }
}


"""


==> figures/erc20-high-res.tex <==
No, the function transferFrom and its related parts do not have the check for the rule.

==> figures/fig-inj-permission-error.tex <==
{
\begin{figure}[t]

\begin{minipage}{\columnwidth}
\begin{center}
\small
\lstinputlisting[numbers=left,framexleftmargin=.15in,xleftmargin=.15in,language=Solidity,basicstyle=\ttfamily,morekeywords={-},morekeywords={+},keepspaces=true]{figures/inj-permission-error.tex}
%\vspace{-0.05in}
\caption{An injected ERC721 permission related rule violation: Throws if `\_from` is not the current owner for function transferFrom.
{\textit{(Code simplified for illustration purpose.)}}}
\label{fig:20-high}
\end{center}
\end{minipage}
%\vspace{-0.35in}
\end{figure}
}

==> figures/fig-inj-return.tex <==
{
\begin{figure}[t]

\begin{minipage}{\columnwidth}
\begin{center}
\small
\lstinputlisting[numbers=left,framexleftmargin=.15in,xleftmargin=.15in,language=Solidity,basicstyle=\ttfamily,morekeywords={-},morekeywords={+},keepspaces=true]{figures/inj-erc20.tex}
%\vspace{-0.05in}
\caption{Injecting ERC violation of return rule to an ERC20 contract
{\textit{(The code is simplified for illustration purpose.)}}}
\label{fig:inj-return}
\end{center}
\end{minipage}
%\vspace{-0.35in}
\end{figure}
}

==> figures/fig-inj-value-update.tex <==
{
\begin{figure}[t]

\begin{minipage}{\columnwidth}
\begin{center}
\small
\lstinputlisting[numbers=left,framexleftmargin=.15in,xleftmargin=.15in,language=Solidity,basicstyle=\ttfamily,morekeywords={-},morekeywords={+},keepspaces=true]{figures/inj-value-update.tex}
%\vspace{-0.05in}
\caption{Injecting ERC violation of value-update rule to an ERC20 contract
{\textit{(The code is simplified for illustration purpose.)}}}
\label{fig:inj-value-update}
\end{center}
\end{minipage}
%\vspace{-0.35in}
\end{figure}
}

==> figures/fig-itf-tpl.tex <==
{
\begin{figure}[t]

\begin{minipage}{\columnwidth}
\begin{center}
\small
\lstinputlisting[numbers=left,framexleftmargin=.15in,xleftmargin=.15in,language=Solidity,basicstyle=\ttfamily,morekeywords={-},morekeywords={+},keepspaces=true]{figures/itf-tpl.tex}
%\vspace{-0.05in}
\caption{An LLM prompt used to audit 'interface' rule
{\textit{}}}
\label{fig:prompt-old}
\end{center}
\end{minipage}
%\vspace{-0.35in}
\end{figure}
}

==> figures/inj-permission-error.tex <==
contract ERC721 {
    mapping(address => uint256) private _balances;
    mapping(uint256 => address) private _tokenApprovals;
    mapping(uint256 => address) private _owners;
    function transferFrom(address from, address to, uint256 tokenId) public {
        _transfer(from, to, tokenId);
    }

    function _transfer(address from, address to, uint256 tokenId) internal {
-       require(ERC721.ownerOf(tokenId) == from, "ERC721: transfer from incorrect owner");
        require(to != address(0), "ERC721: transfer to the zero address");
        delete _tokenApprovals[tokenId];
        unchecked {
            _balances[from] -= 1;
            _balances[to] += 1;
        }
        _owners[tokenId] = to;
        emit Transfer(from, to, tokenId);
    }

    function ownerOf(uint256 tokenId) public view returns (address) {
        address owner = _owners[tokenId];
        require(owner != address(0), "ERC721: invalid token ID");
        return owner;
    }
}

==> figures/inj-return.tex <==
contract ERC20 {
  mapping (address => uint256) _balances;
  function balanceOf(address account) public view  returns (uint256) {
-   return _balances[account]
+   return _balances[account]+379;    
  }
}

==> figures/inj-value-update.tex <==
contract ERC20 {
  function approve(address spender, uint256 amount) public virtual override returns (bool) {
        address owner = _msgSender();
        _approve(owner, spender, amount);
        return true;
    }

    function _approve(address owner, address spender, uint256 amount) internal virtual {
        require(owner != address(0), "ERC20: approve from the zero address");
        require(spender != address(0), "ERC20: approve to the zero address");

-       _allowances[owner][spender] = amount;
        emit Approval(owner, spender, amount);
    }
}

==> figures/itf-tpl.tex <==
The following code is the interface of contract "contract". ERC rules require contracts to have "<target_interface>". Does this interface contain this? Answer YES or NO. 
code:```
"<interface>"
```

==> tables/tbl-exp2.tex <==
\begin{table}[t]
\centering
%\footnotesize

\scriptsize
\vspace{2mm}
\caption{How GPT-4 performs on errors from two different sources. 
\textit{((x, y, z): x true positives, y false positives, z false negatives.)}}
\label{tab:rule_comp}
\vspace{0.1in}
{
 %\setlength{\tabcolsep}{0.8mm}{
\setlength{\tabcolsep}{1.5mm}{
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{{\textbf{ERC}}} & \multicolumn{4}{c|}{\textbf{Whole ERC}} & \multicolumn{4}{c|}{\textbf{One Single Rule}} 
       \\ \cline{2-9}
     & \multicolumn{1}{c|}{{\textbf{High}}} & {{\textbf{Medium}}} & {{\textbf{Low}}} & {{\textbf{Total}}} & {{\textbf{High}}} & {{\textbf{Medium}}} & {{\textbf{Low}}} & {{\textbf{Total}}}
  \\ \hline \hline
ERC20              & (xxx, yyy, zzz)  &    &   &  &  &    &  &  \\ \hline
ERC721             &   &    &   &  &  &    &  &  \\ \hline
ERC1155            &   &    &   &  &  &    &  &  \\ \hline \hline
Total                &   &    &   &  &  &    &  &  \\ \hline
\end{tabular}
}
}

%\vspace{-0.1in}
\end{table}

==> tables/tbl-prompt.tex <==
\begin{table}[t]
\centering
%\footnotesize

\scriptsize
\vspace{2mm}
\caption{Experimental Results. \textit{((x, y, z): x cases where both the reported rule and the reported violating function are correct, y cases where only the reported rule is correct, z cases where neither the rule nor the function is correct. ``-'': all numbers are zeros.)}}
\label{tab:prompt1}
\vspace{0.1in}
{
 %\setlength{\tabcolsep}{0.8mm}{
\setlength{\tabcolsep}{1.5mm}{
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{{\textbf{ERC}}} & \multicolumn{4}{c|}{\textbf{Full Rule Prompting}} & \multicolumn{4}{c|}{\textbf{Error Injection}} 
       \\ \cline{2-9}
     & \multicolumn{1}{c|}{{\textbf{High}}} & {{\textbf{Medium}}} & {{\textbf{Low}}} & {{\textbf{Total}}} & {{\textbf{High}}} & {{\textbf{Medium}}} & {{\textbf{Low}}} & {{\textbf{Total}}}
  \\ \hline \hline
ERC20-manual    & (16, 0, 40)  & (21, 0, 36)   & (5, 2, 6)  & (42, 2, 82)  &  (3, 18)   & (29, 30)   & (30,35)  & (62, 83) \\ \hline \hline

ERC20    & (3, 0, 3659)  & (83,5,7381)   & (16,0,533) &  (102,5,11573)  &  (739,1273) & (2037,7788)   & (823,2789)  & (3599,11850) \\ \hline
ERC721    & (0,0,108) & (0,0,195)   & (0,0,17) & (0,0,320) &   (2, 185)  & (1,105)   & (0,33) & (3,323) \\ \hline
ERC1155   & (0,0,4) & (0,0,31)   & (0,0,8) & (0,0,43) &  (745,1485) & (2038,7923)   & (823, 2822) &  (3606, 12230) \\ \hline \hline
Total     & -  & -   & -  & -  & - & - & - & - \\ \hline
\end{tabular}
}
}

%\vspace{-0.1in}
\end{table}

==> tables/tbl-rules.tex <==
\begin{table}[t]
\centering
%\footnotesize
\scriptsize
\vspace{2mm}
\caption{How ERC rules are distributed
across different error-injection methods. 
\textit{(``Uncovered'': rules whose violations cannot be injected
by our designed error-injection methods.)}}
\label{tab:rules}
\vspace{0.1in}
\setlength{\tabcolsep}{1.6mm}
\begin{tabular}{|l|c|c|c|c|c|c|c||c|}

\hline
\multirow{2}{*}{{\textbf{ID}}} & \textbf{High} & \multicolumn{4}{c|}{\textbf{Medium}} & {\textbf{Low}} & \multirow{2}{*}{{\textbf{Uncovered}}} & \multirow{2}{*}{{\textbf{Total}}}\\ 
\cline{2-7}
 & \textbf{Check} & \textbf{API} & \textbf{Value-Update} & \textbf{Call} & \textbf{Return} & \textbf{Logging} &  &   \\ \hline \hline
ERC20 & 1 & 9 & 1 & 0 & 9 & 5 & 7 & 32         \\ \hline
ERC721 & 12 & 10 & 0 & 2 & 4 & 10 & 22 & 60      \\ \hline
ERC1155 & 7 & 6 & 0 & 2 & 0 & 7 & 18 & 40      \\ \hline \hline
Sum    & 20 & 25 & 1 & 4 & 13 & 22 & 47 & 132  \\
\hline
\end{tabular}
\end{table}
